Vehicular Multi-object Tracking with Persistent Detector Failures

Autonomous vehicles often perceive the environment by feeding sensor data to a learned detector algorithm, then feeding detections to a multi-object tracker that models object motions over time. Probabilistic models of multi-object trackers typically assume that errors in the detector algorithm occur randomly over time. We instead assume that undetected objects and false detections will persist in certain conditions, and modify the tracking framework to account for them. The modifications are tested on a vehicle tracking dataset using a state-of-the-art lidar-based detector, a novel lightweight detector, and a fusion of camera and lidar detectors. For each detector, the persistence modifications notably improve performance and enable the model to outperform baseline trackers.

==> oldmot.tex <==
\section{Tracking}
This section presents the standard probabilistic formulation of multi-object tracking with a single object detector. We focus on the update step of tracking rather than the prediction/propagation step as this step is generally independent of the detector's properties. Hence a single update step is considered, where a hypothesized distribution over the current set of present objects is updated with a set of detections.

\subsection{Single-object Tracking}
Each tracked object is parameterized with a random state $x$. This includes observable features such as the object's location, shape, and class, as well as latent features such as the object's motion. Each detection has a fixed set of values $z$. In the case that a single object is detected, the detection distribution $P(z|x)$ is assumed. Given an object distribution and a detection, as well the assumption that the detection corresponds to this object, the object's distribution can be updated with a simple application of Bayes rule $P(x|z) = \frac{P(x)P(z|x)}{\int_x P(x)P(z|x)}$. In practice, the probability distributions assumed in tracking models are Gaussians, point mixtures, or mixtures of Gaussians. For instance, if the current state distribution is a Gaussian, the updated state distribution can be estimated as a Gaussian using a variant of the Kalman filter.

\subsection{Multi-object Tracking}
\label{subsec_backmot}
Probabilistic multi-object tracking estimates probability distributions over sets of estimated object states $X=\{x_1, \cdots, x_{|X|}\}$. Random sets differ from vector-valued random variables in that they have no intrinsic ordering and their cardinality $|X|$ is also random. A distribution on a set can be written in terms of a cardinality distribution and a set of joint distributions (one for each cardinality).
\begin{equation}
P(X) = P(|X|=K) \sum_{k\leftrightarrow i}{P\left( x_{k:k\rightarrow 1},x_{k:k\rightarrow 2}, \ldots ,x_{k:k\rightarrow K} \right) }
\end{equation}
Where all possible one-to-one mappings of indices $k \in \{ 1,\ldots ,K\}, i \in \{ 1,\ldots ,K\}$ are summed. Most useful multi-object distributions can be described directly without specifying the cardinality or joint distributions. For instance, the multi-Bernoulli distribution specifies a fixed set of $m$ potential objects, each of which have an independent state distribution $p_i(x)$ and an independent probability of existing $r_i$. The probability of existence of each object is also independent of the object's state.
\begin{align}
P(X)&=\mathbbm{1}\left( |X|\leq m\right) \sum_{k\leftrightarrow i}{\prod_i{\left\{ \begin{array}{lr} r_i p_i(x_k) & k\rightarrow i \\ 1-r_i & \emptyset \rightarrow i \end{array}\right\} }} \\
&= \mathbbm{1}\left( |X|\leq m\right)  \sum_{k\leftrightarrow i}{\prod_{k\rightarrow i}{r_i p_i(x_k)} \prod_{\emptyset \rightarrow i}{1-r_i}} \nonumber
\end{align}
In this case, the mapping from $k$ to $i$ is not one-to-one, as some components in the distribution are not matched to realized objects. The null index $\emptyset$ is used for indices with no match. It is clear that a mixture of an arbitrarily high number of these distributions could form any multi-object probability distribution. This is the intuition behind multiple hypothesis tracking, and \cite{tracking_pmbm} derives the tracking update equations with such a mixture. An equivalent but more compact distribution is presented here. This distribution specifies $m$ potential objects, each with independent state distribution $p_k(x)$, and a joint distribution over the existence of objects $R$. The existence of objects are therefore dependent, but are still independent of any object's state.
\begin{align}
&P(X) = \sum_{k\leftrightarrow i} R(k\leftrightarrow i) \prod_{k\rightarrow i}p_i(x_k) \\
&R(k\leftrightarrow i) = \mathbbm{1}\left(|X|\leq m\right) R\left( \mathbbm{1}\left(\emptyset \rightarrow 1\right), \cdots, \mathbbm{1}\left(\emptyset \rightarrow m\right)\right) \nonumber
\end{align}
Finally, a Poisson process is frequently added to models. Its purpose is to specify regions in which an unknown number of objects may exist. In practice, these are objects that have recently entered the sensor view and have not yet been detected, or objects with too uncertain a position to be tracked accurately. Each Poisson process is described by a rate parameter $\kappa_U$ and a single object state distribution $P_U (x)$.
\begin{align} \label{eq_multiplehypothesisdistribution}
P(X) = e^{-\kappa_U} \sum_{k\leftrightarrow i} R(k\leftrightarrow i) \prod_{k\rightarrow i}p_i(x_k) \prod_{k\rightarrow \emptyset} \kappa P_U (x_k)
\end{align}

\subsubsection{Standard Multi-object Measurement Model} \label{subsec_smm}
A multi-object measurement model specifies the probability distribution of a set of detections $Z = \left\{ z_1, \cdots, z_{|Z|}\right\}$ given a current set of objects $X$. The standard model assumes that each object generates at most one measurement. Additionally, the probability that an object generates a measurement is independent of other objects, and the values of a generated measurement are independent of objects that did not generate it. Finally, some measurements may be erroneous and not correspond to any object. These are termed false positives, and are assumed to be generated by a Poisson process. $r_D$ refers to the probability that an object generates some detection, while $P(z|x)$ is the distribution over measurement $z$ given that it was generated by object $x$. $P_F$ and $\kappa_F$ specify the distribution over the set of false measurements.
\begin{align} \label{eq_smmm}
P(Z|X) = e^{-\kappa_F} \sum_{k\leftrightarrow j} \prod_{k\rightarrow j}r_D(x_k) P(z_j|x_k) &\prod_{k\rightarrow \emptyset}{(1-r_D(x_k))} \nonumber \\
&\prod_{\emptyset\rightarrow j} \kappa_F P_F(z_j)
\end{align}
Alternative measurement models consider detectors such that each object has many measurements \cite{mwo_multimeasurement} or handle special cases of interdependence between objects and measurements. The multi-object tracking update step calculates the posterior probability $P(X|Z)$. Given the multiple hypothesis distribution of \eqref{eq_multiplehypothesisdistribution}, the joint distribution of objects and detections is
\begin{align} \label{eq_smjm}
P(X,Z) = \sum_{k\leftrightarrow i} \sum_{k\leftrightarrow j} &e^{-\kappa_F-\kappa_U} R(k\leftrightarrow i) \prod_{k\rightarrow i}p_i(x_k) \nonumber \\
&\prod_{k\rightarrow j}r_D(x_k) P(z_j|x_k) \prod_{k\rightarrow \emptyset}{(1-r_D(x_k))} \nonumber \\
&\prod_{k\rightarrow \emptyset} \kappa_U P_U (x_k) \prod_{\emptyset\rightarrow j} \kappa_F P_F(z_j)
\end{align}
This large expression be modified to fit the form of the object distribution \eqref{eq_multiplehypothesisdistribution} by combining the assignment terms $i$ and $j$ into a single joint term $i,j$. However, mapping true objects $k$ to joint terms $ij$ allows for many mappings that would not occur in the joint distribution. For instance, mapping object 1 to 1,2 and object 2 to 1,3 is impossible, as two different objects $k=2,3$ are mapped to a single potential object $i=1$. These constraints can be handled by introducing an indicator function $A(k\leftrightarrow i,j)$ that contains the assumed constraints on data association.
\begin{align}
A(k\leftrightarrow i,j) = &\prod_i \mathbbm{1} \left( \sum_k  \mathbbm{1}\left( k\rightarrow i,\emptyset\right) + \sum_{k,j} \mathbbm{1}\left( k\rightarrow i,j\right)  \leq 1\right) \nonumber \\
\times &\prod_j \mathbbm{1} \left( \sum_k \mathbbm{1}\left( k\rightarrow\emptyset,j\right) + \sum_{k,i} \mathbbm{1}\left( k\rightarrow i,j\right) \leq 1\right)
\end{align}
Additionally, the relevant expressions can be separated into likelihood constants and posterior distributions over each $x$.
\begin{align}
&P_{i,j}(z_j) = \int_{x} P_i(x)r_D(x)P(z_j|x) \label{eq_matchlik}\\
&P_{i,\emptyset} = \int_{x} P_i(x) (1-r_D(x)) \label{eq_objmisslik} \\
&P_{\emptyset,j}(z_j) = \kappa_F P_F(z_j) + \kappa_U \int_{x} P_U(x)r_D(x)P(z_j|x) \label{eq_msmtmisslik} \\
&P_{\emptyset,\emptyset} = \kappa_U \int_{x} P_U(x)(1-r_D(x)) \label{eq_sproutlik} \\
&P_{i,j}(x|z_j) = \frac{P_i(x)r_D(x)P(z_j|x)}{P_{i,j}(z_j)} \label{eq_matchpost} \\
&P_{i,\emptyset}(x) = \frac{P_i(x) (1-r_D(x))}{P_{i,\emptyset}} \label{eq_objmisspost}\\
&P_{\emptyset,j}(x|z_j) = \frac{P_U(x)r_D(x)P(z_j|x)}{\int_{x} P_U(x)r_D(x)P(z_j|x)} \label{eq_msmtmisspost}\\
&P_{\emptyset,\emptyset}(x) = \frac{P_U(x)(1-r_D(x))}{\int_{x} P_U(x)(1-r_D(x))} \label{eq_sproutpost}
%P_{i\rightarrow j}(z_j) = \left\{ \begin{array}{lr}
%    \int_{x} P_i(x) (1-r_D(x)) & j=\emptyset \\
%    \kappa_F P_F(z_j) + \kappa_U \int_{x} P_U(x)r_D(x)P(z_j|x) & i=\emptyset \\
%     & \text{else}
%\end{array} \right\}
\end{align}
%And the update expression:
%\begin{equation}
%P_{i\rightarrow j}(x_{ij}|z_j) = \left\{ \begin{array}{lr}
%    P_i(x) (1-r_D(x)) & j=\emptyset \\
%    \int_{x} P_T(x)r_D(x)P(z_j|x) & i=\emptyset \\
%    \int_{x} P_i(x)r_D(x)P(z_j|x) & \text{else}
%\end{array} \right\}
%\end{equation}
We collectively refer to these as the multi-object tracking update expressions. Note that they are similar to the measurement likelihood and object update expressions for single-object tracking. The multi-object joint distribution can then be written up to some normalizing constant.
\begin{align} \label{eq_motposterior}
P(X,Z) = \sum_{k\leftrightarrow i,j} &R_+(k\leftrightarrow i,j) \prod_{k\rightarrow i,j} P_{i,j}(x_k|z_j) \prod_{k\rightarrow i,\emptyset} P_{i,\emptyset}(x_k) \nonumber \\
&\prod_{k\rightarrow \emptyset,j} P_{\emptyset,j}(x_k|z_j) \prod_{k\rightarrow \emptyset,\emptyset} P_{\emptyset,\emptyset} P_{\emptyset,\emptyset}(x_k) \\
R_+(k\leftrightarrow i,j) \propto R&(k\leftrightarrow i) A(k\leftrightarrow i,j) \prod_{k\rightarrow i,j} P_{i,j}(z_j) \nonumber \\
&\prod_{k\rightarrow i,\emptyset} P_{i,\emptyset} \prod_{k\rightarrow \emptyset,j} P_{\emptyset,j}(z_j) \prod_{\emptyset\rightarrow j} \kappa_F P_F(z_j)
\end{align}
This form is clearly equivalent to the multiple hypothesis distribution of \eqref{eq_multiplehypothesisdistribution}. The posterior distribution has one potential object for every matching of prior object $i$ and measurement $j$, as well as potential objects corresponding to prior objects that were not detected and to newly detected objects. Two common classes of tracker, multiple hypothesis trackers and PDA/multi-Bernoulli trackers, are specific cases of this distribution and update.

\subsubsection{Data Association and Multi-Sensor Tracking}
As the distributions of each new potential object are simply updated using single-object trackers, the challenge for multiple object tracking is expressing or approximating the updated object existence distribution $R_+(k\leftrightarrow i,j)$. There is no closed-form expression that does not grow in complexity exponentially with each update. However, a wide variety of approximations have been developed to achieve accurate association at high speeds \cite{me_mht, tracking_netflowSSP, mht_blackman, tracking_spline}.

Tracking with multiple detectors can be performed in a sequential fashion by updating with one detector and using the updated distribution as the prior distribution to the next update. If each detector requires complementary information from other detectors to accurately distinguish between objects, or if their detections are correlated (as we are considering), then sequential multi-detector tracking will be inaccurate. Multiple detectors can also update simultaneously by considering joint associations of the tracked objects and all detectors' detections. However, the data association step becomes substantially more challenging with an increasing number of simultaneously-updated sensors.

==> test.tex <==
\section{Vehicle tracking implementation}
%Track-before-Detect
%When high-resolution sensors or multiple sensors are used for object detection, the information returned can be redundant or costly to process. Track-before-detect methods use current estimates of the environment to subselect sensor information to collect or process, with the aim of selecting the information most beneficial to updating the current estimates. Track-before-detect has been used for radar to focus on certain locations [], and has been used in various ways in image-based tracking to only apply the object detection algorithm to part of the image. To our knowledge, it has not been used before for lidar-based 3D tracking. The key challenge of track-before-detect algorithms is an understanding of where unknown or poorly tracked objects may be. For 3D traffic scenes, this requires characterization of the distance and occlusion limitations of the sensor/detector as well as the possibility of moving vehicles entering the visible region.

A hypothesis-oriented multiple-hypothesis tracker is applied to vehicle tracking. Vehicles are considered to occupy 2D rectangles flat along the ground, with height considered unimportant for sensing or tracking. This is often termed a bird's-eye-view (BEV) representation. Vehicles are parameterized by position, orientation, length and width, and speed in the direction of orientation. The sensing vehicle's motion is assumed to be known accurately, so objects are tracked in absolute positions rather than positions relative to the vehicle. Turning is not explicitly modeled, but this model is capable of tracking turning vehicles with steady detections in standard traffic settings. Each detection provides position, orientation, and shape estimates in addition to a score corresponding to the expected probability that this is a genuine detection. While persistent false detections and missed detections are handled as discussed, errors in the detections' estimated values are assumed to be independent across time, objects, and features. In other words, the detector error is assumed to be white noise. This assumption is not necessarily more realistic than that of independent failures, and could be addressed by state augmentation \cite{sensorbiasaugment}. However, short-term errors in position or shape estimation are not considered as significant as detection failures.

A 2D grid of 3-meter square tiles is maintained by the tracker for several functions. The ground surface of each tile is estimated and used to convert between BEV, 3D, and image-space positions. Line-of-sight sensor occlusion is determined for each tile based on the lidar returns, and used to estimate occlusion probability for tracked objects. An occupancy grid \cite{intro_gridmain} is used to model the expected rate and distribution of untracked vehicles entering the system ($\kappa_U$ and $P_U(x)$ in section \ref{subsec_backmot}). The occupancy grid is updated by local mixing at every timestep, simulating the motion of untracked objects and the entry of new objects from outside the field of view. Finally, the importance of performing detection on each tile at each time can be roughly estimated \cite{williams2007information}. This is used to limit computation for one detector, as discussed later.
% The exact parameters are included in Appendix \ref{section_appendixtrackimpl}.

The tracker is tested on the first 10 scenes from the Kitti tracking training dataset. This subset contains 281 unique vehicles with 8307 total annotations. The discussed tracker is denoted as PDFMHT (Persistent Detector Failures in Multiple Hypothesis Tracking) in the following results. % Furthermore, the set of images in the object detection dataset are chosen in a biased fashion, such that detector performance on the object dataset and the tracking dataset will differ.

\subsection{Tracking on Strong Detector}
The tracker is applied to detections from Point-RCNN \cite{pointrcnn}, a deep CNN lidar-based vehicle detector. The same detections were utilized by the tracker in \cite{simpletracking1}, so results from that method are included for comparison. Note that the public benchmark for Kitti only includes tracking in image space, and few methods have stated their performance in terms of BEV or 3D tracking. This is the only easily comparable work with published 3D tracking results; others such as \cite{traffic_monopmbm} do not explain the details of their test data or performance metrics enough for reliable comparison, and lack public code for reproduction.

We report several common MOT performance metrics \cite{data_mot} in Table \ref{tab_strongtrackingresultsT}, calculated as in the MOTChallenge benchmark \cite{data_mot}. Tracked objects are considered to correctly match true objects if the BEV overlap (intersection over union) between the two is greater than 0.5. Note that this is more lax than Kitti's BEV detection criterion of 0.7 overlap, but better considers tracking quality by rewarding correctly-tracked objects even if their precise location or size is not estimated well. Additionally, object detection performance is reported in Table \ref{tab_strongtrackingresultsD}, using the standard Kitti metric of average precision with a 0.7 BEV overlap criterion. This is purely an estimate of how valuable tracking is for improving detection, while the MOT metrics in the former also consider whether objects are tracked consistently over time. As standard with Kitti, the detection metric is calculated on 3 subsets of vehicles ranked by assumed difficulty of detection. The MOT metrics are performed on all annotated vehicles.

\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{PointRCNN+Tracker on Kitti, MOT Performance Metrics}
\label{tab_strongtrackingresultsT}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline \, & MOTA & \# FN & \# FP & \#Switch & MT\% \\
\hline PointRCNN+PDFMHT & 69.4 & 929 & 1607 & 7 & 78 \\
\hline w/o Detectability & 68.2 & 920 & 1612 & 103 & 77 \\
\hline w/o Genuity & 30.9 & 523 & 5085 & 136 & 88 \\
\hline PointRCNN +\cite{simpletracking1} & 65.9 & 1141 & 1673 & 22 & 72 \\
\hline
\end{tabular}
\end{table}
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{PointRCNN+Tracker on Kitti, Detection Performance Metrics}
\label{tab_strongtrackingresultsD}
\begin{tabular}{|c|c|c|c|}
\hline 0.7 IoU & AP Easy & AP Moderate & AP Hard \\
\hline no tracking & 97 & 94 & 93 \\
\hline PDFMHT & 90 & 92 & 92 \\
\hline \cite{simpletracking1} & 88 & 91 & 91 \\
\hline\hline 0.5 IoU & AP Easy & AP Moderate & AP Hard \\
\hline no tracking & 99.1 & 96.7 & 96.2 \\
\hline PDFMHT & 99.2 & 98.9 & 98.9 \\
\hline \cite{simpletracking1} & 98.4 & 97.8 & 97.7 \\
\hline
\end{tabular}
\end{table}

Tracking is not seen to improve detection performance under the standard overlap criterion. We attribute this to the positional requirement being strict enough that synthesizing detections over time is not helpful. On the other hand, the looser overlap requirement shows that tracking definitely improves detection, even when the detection is already quite accurate by most standards. These small improvements in performance may be quite valuable for a reliable perception system. The proposed PDFMHT outperforms the simpler tracker on both overlaps. The tracking metrics show that handling persistent missed detections reduces label switches between objects, while handling persistent false detections drastically reduces false positives. Methods such as \cite{simpletracking1} use score-based cutoffs and that are also resistant to false positives - but PDFMHT still performs better by all metrics.


\subsection{Tracking on Lightweight Lidar Detector}
\subsubsection{Proposed Detector}
\label{subsec_voxeljones}
We propose a simple Viola-Jones-type object detector for vehicular lidar applications, which we refer to as VoxelJones. One of the challenges for classifying on lidar data is deriving useful features from sets of 3D points. Decision trees make binary splits rather than algebraic transformations, so features are not required to be numeric. We select a simple but intuitive and numerous set of binary features. The box of -3 to 3 meters lengthwise with respect to an object's center, -2 to 2 meters widthwise, and .125 to 2.625 meters above the ground is discretized into $0.125$-meter binary voxels (3D cubes). A voxel is positive if at least one lidar point falls within that region of space. Any box-shaped union of voxels may be used as a feature in the classifier. Put another way, each feature is the presence of a lidar detection within some box region of space. There are 30720 voxels within the considered region and over 800 million possible box features. Of course, these features are only calculated if and when used within the classifier.

We use second-order gradient boosting to train weighted regression trees as in \cite{fakes_xgboost}. The decision trees are of depth 3 and so each contain 7 splits and 8 resulting values. A first classifier of 10 trees operates on anchors spaced every 0.5 meters and $\frac{\pi}{8}$ radians. The attentional cascade eliminates 99.8\% of negative inputs, while erroneously eliminating 14\% of positive inputs.%Given that state-of-the-art object detectors on the Kitti dataset only correctly capture 80-85\% of vehicles, we assume that most positive eliminations at this stage would not have been correctly classified by our method anyway.
Positively classified areas are split into anchors spaced at 0.125 meters and $\frac{\pi}{16}$ radians, and further classified with 20 more trees. Additional details such as training, preprocessing, and suppression are discussed in Appendix \ref{appendix_preprocess}.

In addition to inference speed, decision trees and box features have the advantage of interpretability. Appendix \ref{appendix_interpret} includes visual interpretations of the algorithm's parameters and of example input.

\subsubsection{Detector Performance}
The algorithm was trained with the Kitti object detection training dataset, leaving out images corresponding to the first 10 scenes of the Kitti tracking training dataset. Its performance on the Kitti object detection test benchmark is shown in Table \ref{tab_voxeljonesresults}. It is compared to deep network detections from the Kitti public leaderboard. The metric is the same as used in Table \ref{tab_strongtrackingresultsD}, with 0.7 overlap. Algorithm speed is also reported in terms of average detections per second. For most methods, including ours, there is little fluctuation in speed across frames.
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Detector Performance on Kitti BEV Benchmark}
\label{tab_voxeljonesresults}
\begin{tabular}{|c|c|c|c|c|c|}
\hline \, & AP Easy & AP Moderate & AP Hard & FPS & GPU \\
\hline VoxelJones & 65.3 & 54.5 & 49.9 & 6 & N \\
\hline \cite{detect_3DFCN} & 69.4 & 62.5 & 55.9 & 1 & Y \\
\hline \cite{detect_mv3d} & 85.8 & 76.9 & 68.5 & 4 & Y \\
\hline \cite{detect_pointpillars} & 89.3 & 86.1 & 79.8 & 60 & Y \\
\hline \cite{fakes_dnlidarcpu} & -- & -- & 15.4 & 10 & N \\
\hline
\end{tabular}
\end{table}
% on .5 iou 0.898, 0.787, 0.769
Our detection method achieves similar performance to the early deep network \cite{detect_3DFCN}, and superior performance to the only other public method that can be applied in real-time on a CPU \cite{fakes_dnlidarcpu}. However, state-of-the-art detectors are notably better. We next discuss how to track while handling detection errors.

\subsubsection{Tracker Performance}
We report MOT metrics and performance metrics in Tables \ref{tab_fakestrackingresultsT} and \ref{tab_fakestrackingresultsD} respectively.

\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{VoxelJones+Tracker Performance on Kitti, Tracking Metrics}
\label{tab_fakestrackingresultsT}
\begin{tabular}{|c|c|c|c|c|c|}
\hline \, & MOTA & \# FN & \# FP & \#Switch & MT\% \\
\hline PDF-MHT & 53.3 & 2821 & 1057 & 4 & 34 \\
\hline w/o Detectability & 51.5 & 2844 & 1099 & 89 & 33 \\
\hline w/o Genuity & 18.2 & 1511 & 5210 & 71 & 64 \\
\hline 2x Faster & 51.0 & 2885 & 1175 & 7 & 33 \\
\hline
\end{tabular}
\end{table}
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{VoxelJones+Tracker Performance on Kitti, Detection Metrics}
\label{tab_fakestrackingresultsD}
\begin{tabular}{|c|c|c|c|}
\hline .7 IoU & AP Easy & AP Moderate & AP Hard \\
\hline Just Detection & 50 & 47 & 47 \\
\hline PDF-MHT & 42 & 40 & 29 \\
\hline 2x Faster & 39 & 38 & 27 \\
\hline\hline .5 IoU & AP Easy & AP Moderate & AP Hard \\
\hline Just Detection & 85 & 78 & 77 \\
\hline PDF-MHT & 85 & 78 & 77 \\
\hline 2x Faster & 81 & 74 & 73 \\
%\hline \cite{traffic_monopmbm} & 49 & 11 & 20 \\
\hline
\end{tabular}
\end{table}

The tracker is compared to alternate versions without false positive or false negative correlation. Additionally, the tracker is used to subselect a third of the viewed area at every timestep on which to apply the detector. This more than doubles the detector's speed, with the sublinear improvement explained by costly preprocessing and the fact that the selected regions are less likely to be removed in the attentional cascade.

The tracker's performance is highly improved by adding persistent false object reasoning. This is reasonable as the object detector used provides many false positives. Detectability slightly improves performance as with the Point-RCNN detector. The detection performance of VoxelJones is not improved by tracking. However, it is worth noting that the tracker consistently maintained tracks (with very few label switches) without sacrificing detection performance. Additionally, the tracker can be used to increase the detector's speed with only a minor performance penalty. The subselected VoxelJones+tracker pair runs at over 10 updates per second.
